Low-Rank Curvature for Zeroth-Order Optimization in LLM Fine-Tuning

We introduce LOREN, a curvature-aware zeroth-order (ZO) optimization method for fine-tuning large language models (LLMs). Existing ZO methods, which estimate gradients via finite differences using random perturbations, often suffer from high variance and suboptimal search directions. Our approach addresses these challenges by: (i) reformulating the problem of gradient preconditioning as that of adaptively estimating an anisotropic perturbation distribution for gradient estimation, (ii) capturing curvature through a low-rank block diagonal preconditioner using the framework of natural evolution strategies, and (iii) applying a REINFORCE leave-one-out (RLOO) gradient estimator to reduce variance. Experiments on standard LLM benchmarks show that our method outperforms state-of-the-art ZO methods by achieving higher accuracy and faster convergence, while cutting peak memory usage by up to 27.3% compared with MeZO-Adam.

==> subfiles/convergence.tex <==
\section{Convergence Analysis}
\label{sec:supp_convergence}
We make the following assumptions to establish the convergence
property of \loren.

\begin{assumption}[Smoothness] \label{assm:smoothness}
  The objective function $f:\R^{d}\to \R$ is $L$-smooth, meaning
  $\grad{f}$ satisfies
  \[
    \norm{\grad{f}(\vec{x}) - \grad{f}(\vec{y})}\leq
    L\norm{\vec{x}-\vec{y}}\,, \quad \forall \vec{x}, \vec{y}\in \R^{d}\,.
  \]
\end{assumption}
\begin{assumption}[Bounded Variance] \label{assm:bounded_variance}
  The variance of the stochastic gradient $\grad{f}(\vec{x}; \xi)$ is
  bounded by $\sigma^{2}$. That is,
  \[
    \E\left[\norm{\grad{f}(\vec{x};\xi) -
        \grad{f}(\vec{x})}^{2}\right]\leq \sigma^{2}\,, \quad \forall
    \vec{x}\in \R^{d}\,.
  \]
\end{assumption}



\subsection{Proof of Proposition~\ref{prop:grad_gauss_rs}}
We have
\begin{align*}
  \grad{f}_{\epsilon,\mat{\Sigma}}(\vec{x})
  &=\grad_{\vec{x}} \left\{%
    \E_{\vec{u}\sim\mathcal{N}(\vec{0},\mat{\Sigma})}\left[
    f(\vec{x} + \epsilon\vec{u})\right]\right\} \\
  &=(2\pi)^{-d/2}\det(\mat{\Sigma})^{-1/2}\grad_{\vec{x}}\int
    f(\vec{x}+\epsilon\vec{u})
    \exp(-\frac{1}{2}\vec{u}^{\intercal}\mat{\Sigma}^{-1}\vec{u})
    \dd{\vec{u}}\,. \\
  &=(2\pi)^{-d/2}\det(\mat{\Sigma})^{-1/2}\int
    \grad_{\vec{x}} f(\vec{x}+\epsilon\vec{u})
    \exp(-\frac{1}{2}\vec{u}^{\intercal}\mat{\Sigma}^{-1}\vec{u})
    \dd{\vec{u}}\,. \\
  \intertext{Using the change of variables $\vec{z} = \vec{x} +
  \epsilon\vec{u}$, we get }
  &=(2\pi)^{-d/2}\det(\mat{\Sigma})^{-1/2}\int
    \grad_{\vec{z}} f(\vec{z})\exp(-\frac{1}{2\epsilon^{2}}(\vec{z}-\vec{x})^{\intercal}\mat{\Sigma}^{-1}(\vec{z}-\vec{u}))     \abs*{\pdv{\vec{u}}{\vec{z}}} \dd{\vec{z}}\\
  &=(2\pi)^{-d/2}\det(\mat{\Sigma})^{-1/2}\epsilon^{-d}\int\grad_{\vec{z}}f(\vec{z})    
    \exp(-\frac{1}{2\epsilon^{2}}(\vec{z}-\vec{x})^{\intercal}\mat{\Sigma}^{-1}(\vec{z}-\vec{u}))
    \dd{\vec{z}}\,. \\  
  &=\E_{\vec{z}\sim\mathcal{N}(\vec{x},\epsilon^{2}\mat{\Sigma})}\left[%
    \grad{f}(\vec{z})\right] \\
  \intertext{By Stein's identity for the normal distribution, we have }
  &=\E_{\vec{z}\sim\mathcal{N}(\vec{x},\varepsilon^{2}\mat{\Sigma})}\left[%
    \epsilon^{-2}\mat{\Sigma}^{-1}(\vec{z}-\vec{x}) f(\vec{z})\right] \\
  &=(2\pi)^{-d/2}\det(\epsilon^{2}\mat{\Sigma})^{-1/2}\int
    \epsilon^{-2}\mat{\Sigma}^{-1}(\vec{z}-\vec{x})f(\vec{z})
    \exp(-\frac{1}{2\epsilon^{2}}(\vec{z}-\vec{x})^{\intercal}\mat{\Sigma}^{-1}(\vec{z}-\vec{x}))
    \dd{\vec{z}}\,.\\
  \intertext{Applying the change of variables $\vec{u} =
  \frac{\vec{z}-\vec{x}}{\epsilon}$ one more time gives}
  &=(2\pi)^{-d/2}\det(\epsilon^{2}\mat{\Sigma})^{-1/2}\epsilon^{-1}\int
    \mat{\Sigma}^{-1}\vec{u}f(\vec{x}+\epsilon\vec{u})
    \exp(-\frac{1}{2}\vec{u}\mat{\Sigma}^{-1}\vec{u})
    \abs*{\pdv{\vec{z}}{\vec{u}}} \dd{\vec{u}} \\
  &=(2\pi)^{-d/2}\det(\mat{\Sigma})^{-1/2}\varepsilon^{-1}\int
    \mat{\Sigma}^{-1}\vec{u}f(\vec{x}+\epsilon\vec{u})
    \exp(-\frac{1}{2}\vec{u}\mat{\Sigma}^{-1}\vec{u}) \dd{\vec{u}}\\
  &=\E_{\vec{u}\sim\mathcal{N}(\vec{0},\mat{\Sigma})}\left[
    \epsilon^{-1}f(\vec{x}+\epsilon\vec{u}) \mat{\Sigma}^{-1}\vec{u}\right]
\end{align*}
Similarly, we can show that $\grad{f}_{\epsilon,\mat{\Sigma}}(\vec{x})
= -\E_{\vec{u}\sim\mathcal{N}(\vec{0},\mat{\Sigma})}\left[
  \epsilon^{-1}f(\vec{x}-\epsilon\vec{u})
  \mat{\Sigma}^{-1}\vec{u}\right]$. Combining these two completes
the proof. Note that we also have
\[
  \grad{f}_{\epsilon,\mat{\Sigma}}(\vec{x}) =
  \E_{\vec{u}\sim\mathcal{N}(\vec{0},\mat{\Sigma})}\left[ \frac{f(\vec{x}+\epsilon\vec{u}) -
      f(\vec{x})}{\epsilon}\mat{\Sigma}^{-1}\vec{u}  \right]\,.
\]
  


\subsection{Bound on the gradient}
The RLOO gradient estimate is given by
\begin{equation} \label{eq:ca_grad_est}
  \tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x}_t)
  =\frac{1}{\epsilon(K-1)}\sum_{k=1}^{K}\left(f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi) -
    \frac{1}{K}\sum_{j=1}^{K}f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_j;\xi)\right)
  \mat{\Sigma}^{1/2}\vec{u}_k\,. 
\end{equation}
We first show that the gradient estimate in~\eqref{eq:ca_grad_est} is
equal to the preconditioned gradient of random approximation of $f$.
$\tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x}_t)$.
\begin{align*}
  &\hspace{-1.5em}\E_{\vec{u}_{1:K},\xi}\left[\tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x})\right]\\
  &=\E_{\vec{u}_{1:K},\xi}\left[
    \frac{1}{\epsilon(K-1)}\sum_{k=1}^{K}\left(f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi) -
    \frac{1}{K}\sum_{j=1}^{K}f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_j;\xi)\right)
    \mat{\Sigma}^{1/2}\vec{u}_k
    \right]\\
  &=\E_{\vec{u}_{1:K},\xi}\left[
    \frac{1}{\epsilon K}\sum_{k=1}^{K}\left(f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi) -
    \frac{1}{K-1}\sum_{j\neq
    k}f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_j;\xi)\right)
    \mat{\Sigma}^{1/2}\vec{u}_k 
    \right] \\
  &=\frac{1}{\epsilon K}\sum_{k=1}^{K} \E_{\vec{u}_{1:K},\xi}\left[
    f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi)\mat{\Sigma}^{1/2}\vec{u}_k\right]
  \\
  &\qquad 
    -\frac{1}{K-1}\sum_{j\neq  k}\E_{\vec{u}_{1:K},\xi}\left[
    f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_j)\mat{\Sigma}^{1/2}\vec{u}_k\right] \\
  &=\frac{1}{\epsilon K}\sum_{k=1}^{K} \E_{\vec{u}_{1:K},\xi}\left[
    f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi)\mat{\Sigma}^{1/2}\vec{u}_k\right]
  \\
  &\qquad 
    -\frac{1}{K-1}\sum_{j\neq  k} \E_{\vec{u}_{j},\xi}\left[
    f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_j;\xi)\right]\cdot
    \E_{\vec{u}_{k}}\left[\mat{\Sigma}^{1/2}\vec{u}_k\right]\\
  &=\frac{1}{\epsilon K}\sum_{k=1}^{K} \E_{\vec{u}_{1:K},\xi}\left[
    f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}_k;\xi)\mat{\Sigma}^{1/2}\vec{u}_k\right]
  \\
  &=\epsilon^{-1}\E_{\vec{u},\xi}\left[f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u};\xi)
    \mat{\Sigma}^{1/2}\vec{u}\right] \\
  &=
    \E_{\tvec{u},\xi}\left[\frac{f(\vec{x}+\epsilon\tvec{u};\xi)
    -f(\vec{x};\xi)}{\epsilon} \tvec{u}\right] =
    \tilde{\mat{H}}^{-1}\grad{f}_{\epsilon,\mat{\Sigma}}(\vec{x}) \,,
    \quad \tvec{u}\sim\mathcal{N}(\vec{0}, \mat{\Sigma})\,.
\end{align*}
From the first order Taylor approximation of $f$, we have
\[
  f(\vec{x}+\epsilon\mat{\Sigma}^{1/2}\vec{u}) = f(\vec{x}) +
  \epsilon\grad{f}(\vec{x})^{\intercal}\mat{\Sigma}^{1/2}\vec{u} +
  \mathcal{O}(\epsilon^{2})\,.
\]

\paragraph{Bound on the gradient norm} We can bound the norm of gradient
estimate as
\begin{align*}
  \E_{\vec{u}}\left[\norm{\tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x})}^{2}\right]
  &= \E_{\vec{u}}\left[%
    \norm{\mat{\Sigma}^{1/2}\vec{u}\vec{u}^{\intercal}\mat{\Sigma}^{1/2} \grad{f}(\vec{x})
    + \mathcal{O}(\epsilon)}^{2}
    \right] \\
  &\leq 2\E_{\vec{u}}\left[%
    \norm{\mat{\Sigma}^{1/2}\vec{u}\vec{u}^{\intercal}\mat{\Sigma}^{1/2}
    \grad{f}(\vec{x})}^{2}\right]
    + \mathcal{O}(\epsilon^{2}) \\
  &=2\E_{\vec{u}}\left[%
    \grad{f}(\vec{x})^{\intercal}\mat{\Sigma}^{1/2}\vec{u}\vec{u}^{\intercal}
    \mat{\Sigma}\vec{u}\vec{u}^{\intercal}\mat{\Sigma}^{1/2}\grad{f}(\vec{x})\right]
    + \mathcal{O}(\epsilon^{2}) \\
  &=2\E_{\vec{u}}\left[%
    (\vec{u}^{\intercal}\mat{\Sigma}^{1/2}\grad{f}(\vec{x}))^{2}\vec{u}^{\intercal}\mat{\Sigma}\vec{u}
    \right] + \mathcal{O}(\epsilon^{2}) \\
  &=2\Trace(\mat{\Sigma}) \cdot \grad{f}(\vec{x})^{\intercal}\mat{\Sigma}
    \grad{f}(\vec{x}) +
    4\grad{f}(\vec{x})^{\intercal}\mat{\Sigma}^{2}\grad{f}(\vec{x}) +
    \mathcal{O}(\epsilon^{2}) \\
  &\leq 2\left(\Trace(\mat{\Sigma}) + 2\rho^{-1}\right)
    \grad{f}(\vec{x})^{\intercal}\mat{\Sigma}\grad{f}(\vec{x})
    + \mathcal{O}(\epsilon^{2})\,,
\end{align*}
where the last equality is due to Lemma~\ref{lem:grad_norm_usu} and
the last inequality used the fact that the largest eigenvalue of
$\mat{\Sigma}$ is $\rho^{-1}$.
\begin{lemma} \label{lem:grad_norm_usu}
  For $\vec{u}\sim\mathcal{N}(\vec{0}, \mat{I}_d)$, a symmetric
  matrix $\mat{\Sigma}\in \R^{d\times d}$, and a fixed vector
  $\vec{v}\in \R^{d}$, we have
  \[
    \E_{\vec{u}}\left[(\vec{u}^{\intercal}\mat{\Sigma}^{1/2}\vec{v})^{2}\vec{u}\mat{\Sigma}\vec{u}\right]
    =\Trace(\mat{\Sigma}) \cdot \vec{v}^{\intercal}\mat{\Sigma}\vec{v}
    + 2\vec{v}^{\intercal}\mat{\Sigma}^{2}\vec{v}\,.
  \]
\end{lemma}
\begin{proof}
  Let $\vec{g} = \mat{\Sigma}^{1/2}\vec{v}$.
  \begin{align*}
    \E_{\vec{u}}\left[(\vec{u}^{\intercal}\mat{\Sigma}^{1/2}\vec{v})^{2}\vec{u}\mat{\Sigma}\vec{u}\right]
    &=\E\left[\left(\sum_{i=1}^{d}u_ig_i\right)^{2}
      \left(\sum_{k=1}^{d}u_k\sum_{\ell=1}^{d}\Sigma_{k\ell}u_\ell\right)
      \right] \\
    &=\E\left[\left(\sum_{i=1}^{d}\sum_{j=1}^{d}u_iu_jg_ig_j\right)
      \left(\sum_{k=1}^{d}\sum_{\ell=1}^{d}u_ku_\ell\Sigma_{k\ell}\right)\right]\\
    &=\E\left[\sum_{i,j,k,\ell}
      (u_iu_ju_ku_\ell)g_ig_j\Sigma_{k\ell}\right]\\
    &=\sum_{i,j,k,\ell} \E\left[u_iu_ju_ku_\ell\right]
      g_ig_j\Sigma_{k\ell}
    \\
    \intertext{Since the first and third moments of $\mathcal{N}(0, 1)$ are 0, we
    have}
    &=\sum_{i,j,k,\ell} (\delta_{ij}\delta_{k\ell} +
      \delta_{ik}\delta_{j\ell} + \delta_{i\ell}\delta_{jk})g_ig_j\Sigma_{k\ell}\,,
  \end{align*}
  where $\delta_{ij}$ is the Kronecker delta that returns 1 if $i=j$
  and 0 otherwise.
  \begin{enumerate}[label=(\roman*)]
  \item When $\delta_{ij}\delta_{k\ell} = 1$,
    \[
      \sum_{i,j,k,\ell}g_ig_j\Sigma_{k\ell} =
      \sum_{i,k}g_i^{2}\Sigma_{k,k} = \sum_{i}g_i^{2} \cdot
      \Trace(\mat{\Sigma}) = \norm{\vec{g}}^{2}\cdot \Trace(\mat{\Sigma})\,.
    \]
  \item When $\delta_{ik}\delta_{j\ell}=1$,
    \[
      \sum_{i,j,k,\ell}g_ig_j\Sigma_{k\ell} =
      \sum_{i,j}g_ig_j\Sigma_{ij} = \vec{g}^{\intercal}\mat{\Sigma}\vec{g}\,.
    \]
  \item When $\delta_{i\ell}\delta_{jk}=1$,
    \[
      \sum_{i,j,k,\ell}g_ig_j\Sigma_{k\ell} =
      \sum_{i,j}g_ig_j\Sigma_{ji} = \vec{g}^{\intercal}\mat{\Sigma}\vec{g}\,.
    \]
  \end{enumerate}  
  Combining these three cases gives the result.
\end{proof}
For a positive definite matrix $\mat{\Sigma}$, we define $\mat{\Sigma}$-norm of $\vec{x}$ as 
$\norm{\vec{x}}_{\mat{M}} = \sqrt{\vec{x}^\intercal\mat{M}\vec{x}}$.
The $\mat{\Sigma}$-norm of the stochastic gradient is
\begin{align*}
  \E\left[\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}_{\mat{\Sigma}_t}\right]
  &=\E\left[\norm{\grad{f}(\vec{x}_t;\xi_t) +
    \grad{f}(\vec{x}_t)-\grad{f}(\vec{x}_t)}^{2}_{\mat{\Sigma}_t}\right]
  \\
  &\leq 2\norm{\grad{f}(\vec{x}_t)}_{\mat{\Sigma}_t}^{2}
    + 2
    \E\left[\norm{\grad{f}(\vec{x}_t;\xi_t)-\grad{f}(\vec{x}_t)}^{2}_{\mat{\Sigma}_t}\right]\\
  &\leq 2\norm{\grad{f}(\vec{x}_t)}_{\mat{\Sigma}_t}^{2}
    +
    2\rho^{-1}\E\left[\norm{\grad{f}(\vec{x}_t;\xi_t)-\grad{f}(\vec{x}_t)}^{2}\right]\\
  &\leq 2\norm{\grad{f}(\vec{x}_t)}_{\mat{\Sigma}_t}^{2} +
    2\rho^{-1}\sigma^{2}\,.
\end{align*}

\subsection{Proof of Theorem~\ref{thm:convergence}}
From the $L$-smoothness of $f$,
\begin{align*}
  \E_{\vec{u}}\left[f(\vec{x}_{t+1};\xi_{t+1})\right]
  &\leq f(\vec{x}_{t};\xi_t) -\eta_t\E_{\vec{u}}\left[
    \grad{f}(\vec{x}_t;\xi_t)^{\intercal}  \tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x}_t)\right] +
    \frac{L\eta_t^{2}}{2}
    \E_{\vec{u}}\left[\norm{\tvec{g}_{\epsilon,\mat{\Sigma}}(\vec{x}_t)}^{2}\right]
  \\
  &\leq f(\vec{x}_t; \xi_t) -
    \eta_t\norm{\grad{f}(\vec{x}_t; \xi_t)}^{2}_{\mat{\Sigma}}
    + \eta_t\mathcal{O}(\epsilon\norm{\grad{f}(\vec{x}_t; \xi_t)}) \\
  &\qquad
    + 2\eta_t^{2}L(\Trace(\mat{\Sigma}_t) + 2\rho^{-1})\norm{\grad{f}(\vec{x}_t; \xi_t)}_{\mat{\Sigma}_t}^{2} \\
  &\qquad + 2\eta_t^{2}L(\Trace(\mat{\Sigma}_t) +2\rho^{-1})\rho^{-1}\sigma^{2} + \mathcal{O}(\epsilon^{2})\\
  &\leq f(\vec{x}_t; \xi_t)
    -\frac{\eta_t}{2}\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}_{\mat{\Sigma}_t}
    + 2\eta_t^{2}L(\Trace(\mat{\Sigma}) +
    2\rho^{-1})\norm{\grad{f}(\vec{x}_t; \xi_t)}_{\mat{\Sigma}_t}^{2}
  \\
  &\qquad
    + 2\eta_t^{2}L(\Trace(\mat{\Sigma}_t)
    +2\rho^{-1})\rho^{-1}\sigma^{2} + \mathcal{O}(\epsilon^{2})\\
  &=f(\vec{x}_t; \xi_t)-\frac{\eta_t}{2}\left(1 - 4\eta_tL(\Trace(\mat{\Sigma}_t) +
    2\rho^{-1})\right)\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}_{\mat{\Sigma}_t}
  \\
  &\qquad + 2\eta_t^{2}L(\Trace(\mat{\Sigma}_t)2\rho^{-1})
    \rho^{-1}\sigma^{2} + \mathcal{O}(\epsilon^{2})\,. \\
  \intertext{With the choice of $\eta_t = \eta = \frac{1}{8L\sqrt{T}(\max_t
  \Trace(\mat{\Sigma}_t) + 2\rho^{-1})}$, we have}
  &\leq f(\vec{x}_t; \xi_t)-\frac{\eta_t}{4}\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}_{\mat{\Sigma}_t}
  + 2\eta_t^{2}L(\Trace(\mat{\Sigma}_t)+2\rho^{-1})
    \rho^{-1}\sigma^{2} + \mathcal{O}(\epsilon^{2})\,.
\end{align*}
Rearranging the equation yields
\begin{align*}
  \E\left[\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}_{\mat{\Sigma}_t}\right]
  &\leq \frac{4\E\left[f(\vec{x}_t; \xi_t) - f(\vec{x}_{t+1};\xi_{t+1})\right]}{\eta_t}
    + 8\eta_tL(\Trace(\mat{\Sigma}_t) +
    2\rho^{-1})\frac{\sigma^{2}}{\rho}
    + \mathcal{O}(\epsilon^{2})\\
  \intertext{Summing the equations for $t=1, 2, \ldots, T$, we obtain}
  \E\left[\sum_{t=1}^{T}
  \norm{\grad{f}(\vec{x}_t;\xi_t)}_{\mat{\Sigma}_t}^{2}\right]
  &\leq \frac{4\left(f(\vec{x}_1; \xi_1) -
    f(\vec{x}_{T+1};\xi_{T+1})\right)}{\eta}
    +\frac{\sigma^{2}\sqrt{T}}{\rho}
    + \mathcal{O}(T\epsilon^{2}) \\
  &\leq \frac{4\left(f(\vec{x}_1; \xi_1) - f(\vec{x}_{*};\xi_{*})\right)}{\eta}
    +\frac{\sigma^{2}\sqrt{T}}{\rho}
    + \mathcal{O}(T\epsilon^{2})\,. \\
  \intertext{From the above, we get}
  \min_{t=1:T}\E\left[\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}\right]
  &\leq
    \frac{1}{T}\E\left[\sum_{t=1}^{T}\norm{\grad{f}(\vec{x}_t;\xi_t)}^{2}\right]
    \leq \frac{1}{T\alpha_{\min}}\E\left[\sum_{t=1}^{T}
    \norm{\grad{f}(\vec{x}_t;\xi_t)}_{\mat{\Sigma}_t}^{2}\right]\\
  &\leq \frac{4\left(f(\vec{x}_1; \xi_1) - f(\vec{x}_{*};\xi_{*})\right)}{T\eta\alpha_{\min}} +
    \frac{\sigma^{2}}{\sqrt{T}\alpha_{\min}} +
    \mathcal{O}(\epsilon^{2})\\
  &=\frac{32L(\min_t \Trace(\mat{\Sigma}_t) +
    2\rho^{-1})\left(f(\vec{x}_1; \xi_1) -
    f(\vec{x}_{*};\xi_{*})\right)}{\sqrt{T}\alpha_{\min}}
    + \frac{\sigma^{2}}{\sqrt{T}\alpha_{\min}} +
    \mathcal{O}(\epsilon^{2})\,,
\end{align*}
where $\alpha_{\min} = (\rho + \max_t\norm{\vec{a}_t}^{2})^{-1}$ is the smallest
eigenvalue of $\mat{\Sigma}_t$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

